Low Rank Multi-Dictionary Selection at Scale

The sparse dictionary coding framework represents signals as a linear combination of a few predefined dictionary atoms. It has been employed for images, time series, graph signals and recently for 2-way (or 2D) spatio-temporal data employing jointly temporal and spatial dictionaries. Large and over-complete dictionaries enable high-quality models, but also pose scalability challenges which are exacerbated in multi-dictionary settings. Hence, an important problem that we address in this paper is: How to scale multi-dictionary coding for large dictionaries and datasets? We propose a multi-dictionary atom selection technique for low-rank sparse coding named LRMDS. To enable scalability to large dictionaries and datasets, it progressively selects groups of row-column atom pairs based on their alignment with the data and performs convex relaxation coding via the corresponding sub-dictionaries. We demonstrate both theoretically and experimentally that when the data has a low-rank encoding with a sparse subset of the atoms, LRMDS is able to select them with strong guarantees under mild assumptions. Furthermore, we demonstrate the scalability and quality of LRMDS in both synthetic and real-world datasets and for a range of coding dictionaries. It achieves 3X to 10X speed-up compared to baselines, while obtaining up to two orders of magnitude improvement in representation quality on some of the real world datasets given a fixed target number of atoms.

==> tex/7_acknowledgement.tex <==
\section{Acknowledgement}
This research was funded by the NSF SC\&C grant CMMI-1831547. AM was funded by NSF CCF grants CIF-2212327 and CIF-2338855.

==> tex/8_conclude.tex <==
\vsa
\section{Conclusion}
In this paper we introduced \ourmeth, a scalable and accurate method for sparse multi-dictionary coding of 2D datasets. Our approach sub-selects dictionary atoms and employs convex optimization to encode the data using the selected atoms. We provided a theoretical guarantee for the quality of the atom sub-selection for the task of denoising the data. We also demonstrated the quality and scalability of \ourmeth on several real-world datasets and by employing multiple analytical dictionaries. It outperformed state-of-the-art 2D sparse coding baselines by up to $1$ order of magnitude in terms of running time and up to $2$ orders of magnitude in representation quality on some of the real-world datasets. As a future direction, we plan to extend our dictionary selection approach to multi-way data (i.e., tensors) making the core idea applicable to a wider range of problem settings.
